Test like you Train in Implicit Deep Learning

Implicit deep learning has recently gained popularity with applications ranging from meta-learning to Deep Equilibrium Networks (DEQs). In its general formulation, it relies on expressing some components of deep learning pipelines implicitly, typically via a root equation called the inner problem. In practice, the solution of the inner problem is approximated during training with an iterative procedure, usually with a fixed number of inner iterations. During inference, the inner problem needs to be solved with new data. A popular belief is that increasing the number of inner iterations compared to the one used during training yields better performance. In this paper, we question such an assumption and provide a detailed theoretical analysis in a simple setting. We demonstrate that overparametrization plays a key role: increasing the number of iterations at test time cannot improve performance for overparametrized networks. We validate our theory on an array of implicit deep-learning problems. DEQs, which are typically overparametrized, do not benefit from increasing the number of iterations at inference while meta-learning, which is typically not overparametrized, benefits from it.

==> cmdmaths.tex <==
% Ensembles

\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbZ}{\mathbb{Z}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbV}{\mathbb{V}}

\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\calZ}{\mathcal{Z}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calS}{\mathcal{S}}


\renewcommand\qedsymbol{$\blacksquare$}

\newcommand{\train}{{\mathrm{train}}}
\newcommand{\test}{{\mathrm{test}}}
\newcommand{\val}{{\mathrm{val}}}


\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\diag}{\mathbf{diag}}

% Pour avoir les indices en-dessous

\newcommand*{\somme}{\sum\limits}
\newcommand*{\produit}{\prod\limits}
\newcommand*{\limite}{\lim\limits}
\newcommand*{\bsup}{\sup\limits}
\newcommand*{\binf}{\inf\limits}
\newcommand*{\Max}{\max\limits}
\newcommand*{\Min}{\min\limits}
\newcommand*{\integ}{\displaystyle \int}
\newcommand*{\prive}{\setminus}
\newcommand*{\ens}[1]{\left\{#1\right\}}
\newcommand*{\PPCM}{\bigvee\limits}
\newcommand*{\PGCD}{\bigwedge\limits}
\newcommand*{\union}{\bigcup\limits}
\newcommand*{\inter}{\bigcap\limits}

\newcommand*{\ppcm}[2]{#1\vee #2}
\newcommand*{\pgcd}[2]{#1\wedge #2}

\newcommand{\diff}{\mathrm{d}}
\newcommand{\e}{\mathrm{e}}
\renewcommand{\i}{\mathrm{i}}

%Equation hors paragraphe encadrée

\newcommand{\Eenc}[1]{\begin{empheq}[box=\fbox]{equation*}#1\end{empheq}}

%Intervalles

\newcommand{\intff}[2]{\left[#1\,,#2\right]}
\newcommand{\intoo}[2]{\left]#1\,,#2\right[}
\newcommand{\intof}[2]{\left]#1\,,#2\right]}
\newcommand{\intfo}[2]{\left[#1\,,#2\right[}
\newcommand{\intint}[2]{\left\llbracket #1\,, #2 \right\rrbracket}
\newcommand{\E}[1]{\left\lfloor #1 \right\rfloor}

\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\norme}[1]{\left\| #1 \right\|}
\newcommand{\normet}[1]{\left|\left|\left| #1 \right|\right|\right|}


\renewcommand{\vec}[1]{\
\overrightarrow{#1}}
\newcommand{\im}{\mathrm{Im}}
\renewcommand{\ker}{\mathrm{ker}}
\newcommand{\id}{\mathrm{id}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\rg}{\mathrm{rg}}
\newcommand{\Vect}{\mathrm{Vect}}
\newcommand{\Com}{\mathrm{Com}}
\newcommand{\fr}{\mathrm{fr}}
\newcommand{\Sp}[1]{\mathrm{Sp} \pg #1 \pd}

\newcommand{\pg}{\left(}
\newcommand{\pd}{\right)}

\newcommand{\ps}[2]{\left\langle #1\,, #2 \right\rangle}

\newcommand{\Int}[1]{\overset{\circ}{#1}}
\newcommand{\Adh}[1]{\overline{#1}}
